Interactions of Coloured Heavy Stable Particles in Matter

In this paper we present a physics model for the interactions of stable heavy hadrons containing a heavy parton with matter. The model presented is a natural continuation of the work started in hep-ex/0404001. However, changes and generalisations have been made allowing for the description of a broader scope of physics scenarios. As a special case the model is tested on the cases of stable gluino and stop hadrons, thus covering both stable colour triplet and octet states. Conclusions are drawn regarding the phenomenology of these cases including how to distinguish between them.

==> Makefile <==
##
## Makefile for makedvi.pl version 0.31
##
## Makefile for latex documents. Uses the perl script makedvi.pl to
## ensure everything gets compiled.
##
## Written by Thomas Kittelmann (kittel@nbi.dk), Feb. 2003.
##
## Known problems with bibtex: Script does not realise if a \cite{} is
## removed from the tex files. To remove the reference from the
## bibliography, make clean and then make again
##
## version history:
##
##
## version 0.31  Added support for footnpag package.
## version 0.3   Directory is now left in same state as before when
##               making backups.
##               Changed backup naming scheme so alphabetic sorting of
##               a bunch of backups also corresponds to time sorting.
## version 0.22  dvips now outputs to temporary postscript file that is
##               afterwards moved to final ps file. This should prevent
##               gv in 'watch file' mode from giving errors on large
##               files/slow machines.
##               Also made it possible to change title field in ps file
##               (albeit in a on-elegant manner).
## version 0.21  Made it optional for backupremote to keep backup in ./
## version 0.2   Added possibility to only dvips certain pages
##               when making a ps file.
##               Also made file more user friendly by adding more comments.
##               Also implementing automatic copying of backups.
## version 0.1   First numbered version
##
##
###########################################################################
###########################################################################
## Make appropriate changes here:
##

# Name of main tex file:
PROJECT=paper

# Do you have a Table Of Contents?
TOC=FALSE

# Do you have a List Of Figures?
LOF=FALSE

# Do you have a List Of Tables?
LOT=FALSE

# Do you use the package footnpag?
FOOTNPAG=FALSE

# Do you use BibTeX?
BIBTEX=FALSE
# If so, what is the name of the library file?
BIBTEXFILE=rasbib.bib

# Do you use GlossTeX?
GLOSSTEX=FALSE
# If so, what is the name of the library file?
GLOSSTEXFILE=bibgloss.gdf

# Do you use Feynmp?
FEYNMP=TRUE
#IMPORTANT!!: Note that if FEYNMP=TRUE, then all *.mp files are
# considered temporary Feynmp files due for deletion by make clean and
# make realclean (along with any associated .1, .log, .t1 files)
# unless they appear in the following list:
PROTECTEDMPFILES=feynmp.mp

# Project name prefixed to backups
PROJECTID=rm_g4paper
# Places to put backup. A backup is always left in the current working dir.
#*BACKUPLOCATIONS=alf:~/tk_speciale_backup/ fys:~/tk_speciale_backup/ thomask:~/.tk_speciale_backup/
BACKUPLOCATIONS=heppc18:scrlocal/paperbackup lxplus:paperbackup/
#BACKUPLOCATIONS=lscf:/data/users/kittel/tk_speciale_backup/ alf:~/tk_speciale_backup/ fys:~/tk_speciale_backup/ lscf:~/.tk_speciale_backup/
#BACKUPLOCATIONS=lscf:/data/users/kittel/tk_speciale_backup/ alf:~/tk_speciale_backup/ fys:~/tk_speciale_backup/ thomask:~/.tk_speciale_backup/ lscf:~/.tk_speciale_backup/
#Remove copy of backup from current dir after backupremote?
REMOVECOPYFROMPWD=TRUE

#Title field in ps file: (use 'DEFAULT' for default. This is slightly faster)
# (warning: Not all special characters will work as expected)
PSTITLE=G4Paper

###########################################################################
###########################################################################
## It should not be necessary to change anything below this line
## (but do look around to find out what the various targets do).
###########################################################################
###########################################################################


MAKEDVI=./makedvi.pl

#Figure out appropriate arguments for ${MAKEDVI}
ifeq (${TOC},TRUE)
MAKEDVIARG1=usetoc
endif
ifeq (${LOF},TRUE)
MAKEDVIARG2=uselof
endif
ifeq (${LOT},TRUE)
MAKEDVIARG3=uselot
endif
ifeq (${BIBTEX},TRUE)
MAKEDVIARG4=bibtex=${BIBTEXFILE}
endif
ifeq (${GLOSSTEX},TRUE)
MAKEDVIARG5=glosstex=${GLOSSTEXFILE}
endif
ifeq (${FEYNMP},TRUE)
MAKEDVIARG6=usefeynmp
endif
ifeq (${FOOTNPAG},TRUE)
MAKEDVIARG7=usefootnpag
endif
MAKEDVIARGS=${MAKEDVIARG1} ${MAKEDVIARG2} ${MAKEDVIARG3} ${MAKEDVIARG4} ${MAKEDVIARG5} ${MAKEDVIARG6} ${MAKEDVIARG7}

PAGES=""

dvi:
	${MAKEDVI} ${PROJECT} ${MAKEDVIARGS}

#dvips -Pcmz -Pamz  mydoc.dvi -o
ps:dvi
ifeq (${PAGES},"")
	dvips ${PROJECT}.dvi -o .makedvi_ps
else
	dvips ${PROJECT}.dvi -pp ${PAGES} -o .makedvi_ps
endif
ifeq (${PSTITLE},DEFAULT)
	@mv .makedvi_ps ${PROJECT}.ps
else
	@cat .makedvi_ps|sed -e '1,20s/^%%Title:\ ${PROJECT}.dvi/%%Title:\ ${PSTITLE}/1' > .makedvi_ps2
	@mv .makedvi_ps2 ${PROJECT}.ps
	@rm .makedvi_ps
endif

pdf:ps
	ps2pdf ${PROJECT}.ps

ps.gz:ps
	@rm ${PROJECT}.ps.gz
	gzip ${PROJECT}.ps

all:pdf
	@rm ${PROJECT}.ps.gz
	@cp ${PROJECT}.ps dummy_${PROJECT}.ps
	gzip ${PROJECT}.ps
	@mv dummy_${PROJECT}.ps ${PROJECT}.ps

clean:
#remove .aux files associated with .tex files
	@echo removing auxiliary files	
	@for i in *.tex; do bn=`basename $$i .tex`; rm -f $$bn.aux ; done
#remove .log file
	rm -f ${PROJECT}.log
#remove feynmp files
ifeq (${FEYNMP},TRUE)
	@echo removing feynmp files	
	@for i in *.mp; do bn=`basename $$i .mp`; protected=`echo ${PROTECTEDMPFILES} |grep $$bn.mp`; length=`expr length "$$protected"`; if [ "$$length" -eq "0" ]; then rm -f $$bn.mp $$bn.1 $$bn.log $$bn.t1; fi; done
endif
#remove toc file
ifeq (${TOC},TRUE)
	rm -f ${PROJECT}.toc
endif
#remove lof file
ifeq (${LOF},TRUE)
	rm -f ${PROJECT}.lof
endif
#remove lot file
ifeq (${LOT},TRUE)
	rm -f ${PROJECT}.lot
endif
#remove footnpag file
ifeq (${FOOTNPAG},TRUE)
	rm -f ${PROJECT}.fot
endif
#remove bibtex files
ifeq (${BIBTEX},TRUE)
	rm -f ${PROJECT}.blg
	rm -f ${PROJECT}.bbl
endif
#remove glosstex files
ifeq (${GLOSSTEX},TRUE)
	rm -f ${PROJECT}.glo
	rm -f ${PROJECT}.glx
	rm -f ${PROJECT}.gxg
	rm -f ${PROJECT}.gxs
	rm -f ${PROJECT}.ilg
endif
#remove various files
	rm -f texput.log
	rm -f core
	rm -f *~ .*~
	rm -fr .makedvi*
	rm -f nohup.out
	rm -f missfont.log

realclean:clean
	rm -f ${PROJECT}.dvi
	rm -f ${PROJECT}.ps
	rm -f ${PROJECT}.ps.gz
	rm -f ${PROJECT}.pdf

#backup:realclean
backup:
	@echo Making backup
	@rm -rf .makedvibackup/
	@mkdir .makedvibackup/
	@makedvidate=`date +'%y%m%d_%Hh%Mm'`;\
	makedvipwd=`pwd`;\
	makedvithisdir=`basename $$makedvipwd`;\
	mkdir .makedvibackup/$$makedvithisdir/;\
	cp -pr * .makedvibackup/$$makedvithisdir/;\
	rm -f .makedvibackup/$$makedvithisdir/${PROJECTID}_backup_*.tgz;\
	cd .makedvibackup/$$makedvithisdir/;make realclean;\
        cd ../; tar cvzf ../${PROJECTID}_backup_$$makedvidate.tgz $$makedvithisdir/
	@rm -rf .makedvibackup/

backupremote:backup
	@makedvidate=`date +'%y%m%d_%Hh%Mm'`;\
	for i in ${BACKUPLOCATIONS}; do\
	echo Placing copy at $$i;\
	scp ${PROJECTID}_backup_$$makedvidate.tgz $$i/;\
	done
ifeq (${REMOVECOPYFROMPWD},TRUE)
	@echo Removing copy from present working directory
	@makedvidate=`date +'%y%m%d_%Hh%Mm'`;\
	rm -f ${PROJECTID}_backup_$$makedvidate.tgz
endif

br:backupremote

